On Dynamics of Integrate-and-Fire Neural Networks with Conductance Based Synapses

We present a mathematical analysis of a networks with Integrate-and-Fire neurons and adaptive conductances. Taking into account the realistic fact that the spike time is only known within some \textit{finite} precision, we propose a model where spikes are effective at times multiple of a characteristic time scale $\delta$, where $\delta$ can be \textit{arbitrary} small (in particular, well beyond the numerical precision). We make a complete mathematical characterization of the model-dynamics and obtain the following results. The asymptotic dynamics is composed by finitely many stable periodic orbits, whose number and period can be arbitrary large and can diverge in a region of the synaptic weights space, traditionally called the "edge of chaos", a notion mathematically well defined in the present paper. Furthermore, except at the edge of chaos, there is a one-to-one correspondence between the membrane potential trajectories and the raster plot. This shows that the neural code is entirely "in the spikes" in this case. As a key tool, we introduce an order parameter, easy to compute numerically, and closely related to a natural notion of entropy, providing a relevant characterization of the computational capabilities of the network. This allows us to compare the computational capabilities of leaky and Integrate-and-Fire models and conductance based models. The present study considers networks with constant input, and without time-dependent plasticity, but the framework has been designed for both extensions.

==> F1cdef.tex <==
%
%
%%%%%%%%%%%%%%%%%%%% Cas 1cdef
\begin{figure}[ht!]
\begin{center}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/current.cdef.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/gamma.cdef.eps}

\vspace{0.5cm}

\includegraphics[height=5cm,width=5cm,clip=false]{Figures/distance.cdef.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/spike-interval.cdef.eps}
\vspace{0.5cm}
\caption{Fig. \ref{Fcdef}a, average current $I$; \ref{Fcdef}b, $\left<\gamma \right>$; \ref{Fcdef}c, $\log(\dAS)$;  \ref{Fcdef}d, average spike
interval, for $\sigma \in [0.01:10]$ $\tau_L \in [10-40] ms$. }
\label{Fcdef}\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
%



==> F1cdf.tex <==
%
%%%%%%%%%%%%%%%%%%%% Cas 1cdf
\begin{figure}[ht!]
\begin{center}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/current.cdf.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/gamma.cdf.eps}

\vspace{0.5cm}

\includegraphics[height=5cm,width=5cm,clip=false]{Figures/distance.cdf.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/spike-interval.cdf.eps}
\vspace{0.5cm}
\caption{Fig. \ref{Fcdf}a, average current $I$; \ref{Fcdf}b, $\left<\gamma \right>$; \ref{Fcdf}c, $\log(\dAS)$;  \ref{Fcdf}d, average spike
interval, for $\sigma \in [0.01:1]$ $\tau_L \in [10-40] ms$. }
\label{Fcdf}\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%



==> F1gb.tex <==
%
%%%%%%%%%%%%%%%%%%%% Cas 1gb
\begin{figure}[ht!]
\begin{center}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/current.gb.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/gamma.gb.eps}

\vspace{0.5cm}

\includegraphics[height=5cm,width=5cm,clip=false]{Figures/distance.gb.eps}
\includegraphics[height=5cm,width=5cm,clip=false]{Figures/spike-interval.gb.eps}
\vspace{0.5cm}
\caption{Fig. \ref{Fgb}a, average current $I$; \ref{Fgb}b, $\left<\gamma \right>$; \ref{Fgb}c, $\log(\dAS)$;  \ref{Fgb}d, average spike
interval, for $\sigma \in [0.01:1]$ $\tau_L \in [0-1] ms$. }
\label{Fgb}\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
%

